GenVDM: Generating Vector Displacement Maps From a Single Image

We introduce the first method for generating Vector Displacement Maps (VDMs): parameterized, detailed geometric stamps commonly used in 3D modeling. Given a single input image, our method first generates multi-view normal maps and then reconstructs a VDM from the normals via a novel reconstruction pipeline. We also propose an efficient algorithm for extracting VDMs from 3D objects, and present the first academic VDM dataset. Compared to existing 3D generative models focusing on complete shapes, we focus on generating parts that can be seamlessly attached to shape surfaces. The method gives artists rich control over adding geometric details to a 3D shape. Experiments demonstrate that our approach outperforms existing baselines. Generating VDMs offers additional benefits, such as using 2D image editing to customize and refine 3D details.

==> figs/rebut_comparison.tex <==

\begin{figure}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{figs/rebuttal_comparison.png}
   \caption{Top (left to right): optimization with sample grid sizes of 100, 200, 400, 800.
   Bottom (left to right): optimization with 200, 500, 1200, 2000 steps.}
   \label{fig:rebuttal:comparison}
\end{figure}



==> figs/rebuttal_tripoai.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{figs/tripoai.pdf}
   \caption{Qualitative comparison with Tripo AI. Note that the nose generated by Tripo AI has incorrect four-fold symmetry (left to right as well as front to back).}
   \label{fig:rebuttal:tripoai}
\end{figure}
